Modern Random Access for Satellite Communications

The present PhD dissertation focuses on modern random access (RA) techniques. In the first part an slot- and frame-asynchronous RA scheme adopting replicas, successive interference cancellation and combining techniques is presented and its performance analysed. The comparison of both slot-synchronous and asynchronous RA at higher layer, follows. Next, the optimization procedure, for slot-synchronous RA with irregular repetitions, is extended to the Rayleigh block fading channel. Finally, random access with multiple receivers is considered.

==> chapter3/4-Implementation_examples/Implementation_examples.tex <==
\section{Implementation Examples}

\begin{itemize}
\item CRDSA has an implementation.
\item ZigZag with SDR.
\end{itemize}


==> chapter4/9-Acknowledgments/Acknowledgements.tex <==
\section{Acknowledgements}

==> chapter4/sections/acronyms.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% abbreviations.bib
%%%
%%% \acresetall resets all acronyms to not used. Useful after the abstract to redefine all acronyms in the introduction.
%%% \acf{label} Full: written out form with acronym in parentheses, irrespective of previous use
%%% \acs{label} acronym form, irrespective of previous use
%%% \acl{label} written out form without following acronym
%%% \acp{label} plural form of acronym by adding an s. \acfp. \acsp, \aclp work as well.
%%% \acs{label} Short: short version of the acronym
%%% \acfp, acsp aclp acfi acused acsu aclu
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{acronym}
% A
\acro{A/A}{air-to-air}%
\acro{A-EXEC}{auto execute COCR service}%
\acro{AAC}{airline administrative control}%
\acro{ACK}{acknowledgement}%
\acro{ACP}{aeronautical communications panel}%
\acro{AF}{assured forwarding}%
\acro{AL}{application layer}%
\acro{ANSP}{air navigation service provider}%
\acro{AOC}{airline operational control}%
\acro{APC}{air passenger communication}%
\acro{APT}{airport}%
\acro{ATC}{air traffic control}%
\acro{ATI}{access technology independent}%
\acro{ATM}{air traffic management}%
\acro{ATN}{aeronautical telecommunication network}%
\acro{ATN/IPS}{aeronautical telecommunication network / internet protocol suite}%
\acro{ATN/OSI}{aeronautical telecommunication network / open systems interconnection reference model}%
\acro{ATS}{air traffic services}%
\acro{ATSC}{air traffic service communication}%
\acro{AVBDC}{absolute volume based dynamic capacity}%
\acro{AWGN}{additive white gaussian noise}%
% B
\acro{BB}{bandwidth broking} %
\acro{BBFRAME}{baseband frame}%
\acro{BE}{best effort}%
\acro{BER}{bit error rate}%
\acro{BGAN}{broadband global area network}%
\acro{BSM}{broadband satellite multimedia}%
% C
\acro{CA}{constrained architecture}%
\acro{CAC}{connection admission Control}%
\acro{CC}{congestion control}%
\acro{CDF}{cumulative distribution function}
\acro{CDMA}{code divison multiple access}%
\acro{CLNP}{connectionless networking protocol}%
\acro{CLTP}{connectionless transport protocol}%
\acro{CoA}{care of address}%
\acro{CoS}{class of service}%
\acro{COCR}{communications operating concept and requirements for the future radio system}%
\acro{COTP}{connection oriented transport protocol}%
\acro{COTS}{commercial-off-the-shelf}%
%%\acro{CRA}{Constant Rate Assignment}%
\acro{CRA-CC}{CRA-convolutional code}%
\acro{CRA-SH}{CRA-shannon bound}%
\acro{CRA}{contention resolution ALOHA}%
\acro{CRC}{cyclic redundancy check}%
\acro{CRDSA}{contention resolution diversity slotted ALOHA}%
\acro{CRDSA++}{contention resolution diversity slotted ALOHA++}%
\acro{CS}{class selector}%
\acro{CSA}{coded slotted ALOHA}%
\acro{CSMA}{carrier sense multiple access}%
% D
\acro{DAMA}{demand assigned multiple access}%
\acro{DiffServ}{differentiated services}%
\acro{DoD}{department of defence}%
\acro{DSA}{diversity slotted ALOHA}%
\acro{DSCP}{diffServ code point}%
\acro{DVB}{digital video broadcasting}%
\acro{DVB-RCS+M}{digital video broadcasting - return channel via satellite mobility}%
\acro{DVB-RCS}{digital video broadcasting - return channel via satellite}%
\acro{DVB-S2}{digital video broadcasting - second generation}%
\acro{DVB-S2/RCS}{digital video broadcasting - second generation / return channel via satellite}%
% E
\acro{ECN}{explicite congestion notification}%
\acro{ECRA}{enhanced contention resolution ALOHA}%
\acro{ECRA-SC}{ECRA selection combining}
\acro{ECRA-MRC}{ECRA maximal ratio combining}
\acro{ECTL}{eurocontrol}%
\acro{EF}{expedited forwarding}%
\acro{EGD}{equal-gain diversity}
\acro{ENR}{en-route}%
\acro{ES}{end system}%
\acro{ESA}{European space agency}%
\acro{ETSI}{European telecommunications standards institute}%
\acro{ETSI-BSM}{European telecommunications standards institute - broadband satellite multimedia}%
% F
\acro{FAA}{federal aviation administration}%
\acro{FCA}{free capacity assignment}%
\acro{FDM}{frequency division multiplexing}%
\acro{FDMA}{frequency division multiple access}%
\acro{FEC}{forward error correction}%
\acro{FET}{first entry times}%
\acro{FL}{forward link}%
% G
\acro{GEO}{geostationary orbit}%
\acro{GIG}{global information grid}%
\acro{GSE}{generic stream encapsulation}%
% H
\acro{HA}{home agent}%
\acro{HF}{high frequency}%
% I
\acro{IC}{interference cancellation}%
\acro{ICAO}{international civil aviation organization}%
\acro{IETF}{internet engineering task force}%
\acro{IntServ}{integrated services}%
\acro{IP}{internet protocol}%
\acro{IPS}{internet protocol suite}%
\acro{IPSec}{IP security}%
\acro{IRCRA}{irregular repetition contention resolution ALOHA}%
\acro{IRSA}{irregular repetition slotted ALOHA} %
\acro{IS}{intermediate system}%
\acro{IS-IS-TE}{intermediate system to intermediate system extension for traffic engineering}%
\acro{ISI}{input stream identifier}%
\acro{ISO/OSI}{international organization for standardization/open systems interconnection}%
% K
\acro{Ku}{kurz-under}%
\acro{Ka}{kurz-above}%
% L
\acro{LAE}{link access equipment}%
\acro{LAN}{local area network}%
\acro{LD}{low density}%
\acro{LDACS}{L-band digital aeronautical communication system}%
\acro{L-DACS}{L-band digital aeronautical communication system}%
\acro{LDPC}{low density parity check codes}%
\acro{LEO}{low earth orbit}%
% M
\acro{M2M}{machine-to-machine}
\acro{MAC}{medium access}%
\acro{MCAST}{multicast}%
\acro{MF-TDMA}{multifrequency time division multiple access}%
\acro{MH}{mobile host}%
\acro{MIHF}{Media independent handover function}%
\acro{MLPP}{multi level priority preemption}%
\acro{Mode-S}{mode-select}%
\acro{MPE}{multi protocol encapsulation}%
\acro{MPEG2-TS}{MPEG2 - transport stream}%
\acro{MPLS}{multi protocol label switching}%
\acro{MRC}{maximal-ratio combining}
% N
\acro{NCC}{network control centre}%
\acro{NET}{network connectivity}
\acro{NEWSKY}{NEtWorking the SKY for aeronautical communications}%
\acro{NOC}{non-operational communication}%
\acro{NSIS}{next steps in signalling}%
% O
\acro{OC}{operational communication}%
\acro{ORP}{oceanic, remote and polar}%
\acro{OSI}{open systems interconnection}%
\acro{OSPF}{open shortes path first}%
% P
\acro{PDF}{probability density function}%
\acro{PCE}{predictive capacity estimation}%
\acro{PCN}{pre-congestion notification}%
\acro{PDU}{protocol data unit}%
\acro{PEP}{performance enhancing proxy}%
\acro{PER}{packet error rate}%
\acro{PID}{packet identifier}%
\acro{PLFRAME}{physical layer frame}%
\acro{PLR}{packet loss rates}%
% Q
\acro{QoS}{quality of service}%
\acro{QoS-PRN}{QoS private relay nodes}%
\acro{QoS-RN}{QoS-relay nodes}%
% R
\acro{RA}{random access}%
\acro{RBDC}{rate based dynamic capacity}%
\acro{RCB}{random coding bound}%
\acro{RCS}{return channel via satellite}%
\acro{RCS+M}{return channel via satellite plus mobility}%
\acro{RF}{radio frequency}%
\acro{RFC}{request for comments}%
\acro{RL}{return link}%
\acro{RM}{resource management}%
\acro{RN}{relay nodes}%
\acro{RRM}{radio resource management}%
\acro{RS}{reed solomon}%
\acro{RSVP}{resource reservation protocol}%
\acro{RTT}{round trip time}%
% S
\acro{SA}{slotted ALOHA}%
\acro{SANDRA}{seamless aeronautical networking through integration of data links, radios and antennas}%
\acro{SB}{Shannon bound}%
\acro{S2}{second generation}%
\acro{SC}{selection combining}
\acro{SESAR}{single European sky ATM research}%
\acro{SF}{superframe}%
\acro{SIC}{successive interference cancellation}%
\acro{SLS}{service level specification}%
\acro{SNDCF}{subnetwork dependent convergence function}%
\acro{SNIR}{signal-to-noise and interference ratio}%
\acro{SNR}{signal-to-noise ratio}%
\acro{SWIM}{system wide information management}%
\acro{SYN}{synchronization}%
\acro{SYNC}{synchronization}%
% T
\acro{TCP}{transport control protocol}%
\acro{TCP/IP}{transport control protocol / internet protocol suite}%
\acro{TDMA}{time division multiple access}%
\acro{TE}{traffic engineering}%
\acro{TI}{technology independent}%
\acro{TI-SAP}{technology independent - service access point}%
\acro{TD}{technology dependent}%
\acro{TL}{transport layer}%
\acro{TMA}{terminal maneuvering area}%
\acro{ToS}{type of service}%
% U
\acro{UCA}{unconstrained architecture}%
\acro{UDP}{user datagram protocol}%
% V
\acro{VBDC}{volume based dynamic capacity}%
\acro{VDL}{VHF digital mode}%
\acro{VHF}{very high frequency}%
\acro{VoIP}{voice over IP}%
\acro{VPN}{virtual private networks}%
% W
\acro{WG}{working group}%
\acro{WiMAX}{worldwide interoperability for microwave access}%
% X
\acro{XFECFRAME}{forward error correction frame}%
\end{acronym}

\makeatletter
\newif\ifAC@uppercase@first
\def\Aclp#1{\AC@uppercase@firsttrue\aclp{#1}\AC@uppercase@firstfalse}
\def\AC@aclp#1{%
  \ifcsname fn@#1@PL\endcsname
    \ifAC@uppercase@first
      \expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname
    \else
      \csname fn@#1@PL\endcsname
    \fi
  \else
    \AC@acl{#1}s
  \fi 
}
\edef\AC@uppercase@write{\string\ifAC@uppercase@first\string\expandafter\string\MakeUppercase\string\fi\space}
\def\AC@acrodef#1[#2]#3{%
  \@bsphack
  \protected@write\@auxout{}{%
    \string\newacro{#1}[#2]{\AC@uppercase@write #3}%
  }\@esphack
}
\def\Acl#1{\AC@uppercase@firsttrue\acl{#1}\AC@uppercase@firstfalse}
\makeatother


==> chapter4/sections/acronyms2.tex <==
% A
\DeclareAcronym{AWGN}{short = AWGN ,long = additive white Gaussian noise}
\DeclareAcronym{ACRDA}{short = ACRDA ,long = asynchronous contention resolution diversity ALOHA}
% B
% C
\DeclareAcronym{CDF}{short = CDF ,long = cumulative distribution function}
\DeclareAcronym{CRA-CC}{short = CRA-CC ,long = CRA-convolutional code}
\DeclareAcronym{CRA-SH}{short = CRA-SH ,long = CRA-shannon bound}
\DeclareAcronym{CRA}{short = CRA ,long = contention resolution ALOHA}
\DeclareAcronym{CRDSA}{short = CRDSA ,long = contention resolution diversity slotted ALOHA}
\DeclareAcronym{CRDSA++}{short = CRDSA++ ,long = contention resolution diversity slotted ALOHA++}
\DeclareAcronym{CRI}{short = CRI ,long = contention resolution interval}
\DeclareAcronym{CSA}{short = CSA ,long = coded slotted ALOHA}
\DeclareAcronym{CSI}{short = CSI ,long = channel state information}
% D
\DeclareAcronym{DAMA}{short = DAMA ,long = demand assigned multiple access}
\DeclareAcronym{DSA}{short = DSA ,long = diversity slotted ALOHA}
% E
\DeclareAcronym{ECRA}{short = ECRA ,long = enhanced contention resolution ALOHA}
\DeclareAcronym{ECRA-SC}{short = ECRA-SC ,long = ECRA selection combining}
\DeclareAcronym{ECRA-MRC}{short = ECRA-MRC ,long = ECRA maximal-ratio combining}
\DeclareAcronym{EGC}{short = EGC ,long = equal-gain combining}
% F
\DeclareAcronym{FEC}{short = FEC ,long = forward error correction}
% G
\DeclareAcronym{GEO}{short = GEO ,long = geostationary orbit}
% H
% I
\DeclareAcronym{IC}{short = IC ,long = interference cancellation}
\DeclareAcronym{IRCRA}{short = IRCRA ,long = irregular repetition contention resolution ALOHA}
\DeclareAcronym{IRSA}{short = IRSA ,long = irregular repetition slotted ALOHA}
% K
% L
\DeclareAcronym{LDPC}{short = LDPC ,long = low density parity check}
% M
\DeclareAcronym{M2M}{short = M2M ,long = machine-to-machine}
\DeclareAcronym{MAC}{short = MAC ,long = medium access}
\DeclareAcronym{MF}{short = MF ,long = matched filter}
\DeclareAcronym{MF-TDMA}{short = MF-TDMA ,long = multi-frequency time division multiple access}
\DeclareAcronym{MRC}{short = MRC ,long = maximal-ratio combining}
\DeclareAcronym{MUD}{short = MUD ,long = multiuser detection}
% N
% O
% P
\DeclareAcronym{PDF}{short = PDF ,long = probability density function}
\DeclareAcronym{PER}{short = PER ,long = packet error rate}
\DeclareAcronym{PLR}{short = PLR ,long = packet loss rate}
% Q
% R
\DeclareAcronym{RA}{short = RA ,long = random access}
\DeclareAcronym{RCB}{short = RCB ,long = random coding bound}
\DeclareAcronym{RTT}{short = RTT ,long = round trip time}
% S
\DeclareAcronym{SA}{short = SA , long = slotted ALOHA}
\DeclareAcronym{SB}{short = SB ,long = Shannon bound}
\DeclareAcronym{SC}{short = SC ,long = selection combining}
\DeclareAcronym{SIC}{short = SIC ,long = successive interference cancellation}
\DeclareAcronym{SNIR}{short = SNIR ,long = signal-to-noise and interference ratio}
\DeclareAcronym{SINR}{short = SINR ,long = signal-to-interference and noise ratio}
\DeclareAcronym{SNR}{short = SNR ,long = signal-to-noise ratio}
% T
\DeclareAcronym{TDMA}{short = TDMA ,long = time division multiple access}
% U
\DeclareAcronym{UCP}{short = $\Code$-UCP ,long = $\Code$-unresolvable collision pattern}
% V
\DeclareAcronym{VF}{short = VF ,long = virtual frame}
% W
% X
% Y
% Z


==> chapter4/sections/displaynotation.tex <==

\cleardoublepage

\section*{Notation}


\bigskip

\begin{center}
\begin{tabular}{ l l l}
\hline \hline
$\load$ & \verb;\load; & Load \\
$\tp$ & \verb;\tp; & Throughput \\
$\se$ & \verb;\se; & Spectral Efficiency \\
$\plr$ & \verb;\plr; & Packet Loss Rate \\
$\rate$ & \verb;\rate; & Rate \\
$\maxRate$ & \verb;\maxRate; & Maximum Rate allowed\\
$\mutInf$ & \verb;\mutInf; & Mutual information\\
$\rvDec$ & \verb;\rvDec; & r.v. denoting the outcome of the decoding process\\
$\capacity$ & \verb;\capacity; & Capacity \\
$\capacitySC$ & \verb;\capacitySC; & Capacity selection combinig\\
$\capacityMRC$ & \verb;\capacityMRC; & Capacity maximal-ratio combining\\
$\refCap$ & \verb;\refCap; & Reference Capacity of the Gaussian MAC \\
$\maxCap$ & \verb;\maxCap; & Maximum Capacity \\
$\maxSe$ & \verb;\maxSe; & Maximum spectral efficiency \\
$\normCap$ & \verb;\normCap; & Normalized capacity \\
\\
$\dg$ & \verb;\dg; & Number of replicas per user, i.e. degree \\
\\
$\fraLen$ & \verb;\fraLen; & VF duration \\
$\pkLen$ & \verb;\pkLen; & Packet duration \\
$\symLen$ & \verb;\symLen; & Symbol duration \\
\hline \hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{ l l l}
\hline \hline
$\fraTp$ & \verb;\fraTp; & Duration of VF in packets durations \\
$\VFStart$ & \verb;\VFStart; & Delay w.r.t. the VF start \\
$\RefTime$ & \verb;\RefTime; & User delay w.r.t. the common reference time \\
$\Wind$ & \verb;\Wind; & Decoder window size \\
$\WindSh$ & \verb;\WindSh; & Decoder window shift \\
\\
$\numUs$ & \verb;\numUs; & number of user/transmission terminals \\
$\numSym$ & \verb;\numSym; & number of symbols in a packet/replica \\
$\numBit$ & \verb;\numBit; & number of information bits per packet/replica \\
\\
$\rx$ & \verb;\rx; & received signal \\
$\rxVec$ & \verb;\rxVec; & vector of received samples/symbols \\
$\tx$ & \verb;\tx; & transmitted signal \\
$\txVec$ & \verb;\txVec; & vector of transmitted samples/symbols \\
$\noise$ & \verb;\noise; & noise signal \\
$\noisePr$ & \verb;\noisePr; & white Gaussian process \\
$\noiseVec$ & \verb;\noiseVec; & vector of noise samples \\
$\noiseVar$ & \verb;\noiseVar; & noise variance \\
$\intVal$ & \verb;\intVal; & interference random variable \\
$\intVec$ & \verb;\intVec; & vector of interference samples \\
$\intNum$ & \verb;\intNum; & number of interferers \\
$\ch$ & \verb;\ch; & channel amplitude \\
$\symVal$ & \verb;\symVal; & value of the transmitted symbol \\
$\pulse$ & \verb;\pulse; & pulse shape raised cosine filter \\
$\pulseRoot$ & \verb;\pulseRoot; & pulse shape root raised cosine filter \\
\hline \hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{ l l l}
\hline \hline
$\tm$ & \verb;\tm; & time \\
$\epoch$ & \verb;\epoch; & epoch \\
$\freq$ & \verb;\freq; & frequency \\
$\phase$ & \verb;\phase; & phase \\
\\
$\user$ & \verb;\user; & user index \\
$\replica$ & \verb;\replica; & replica index \\
$\sym$ & \verb;\sym; & symbol index \\
\\
$\usPw$ & \verb;\usPw; & useful received power \\
$\PwAg$ & \verb;\PwAg; & Aggregated recevied power \\
$\usPwTx$ & \verb;\usPwTx; & User transmission power \\
$\noisePw$ & \verb;\noisePw; & noise power \\
$\noiseSD$ & \verb;\noiseSD; & single-sided noise power spectral density \\
$\intPw$ & \verb;\intPw; & interference power \\
$\sinr$ & \verb;\sinr; & \ac{SINR} \\
$\sinrVec$ & \verb;\sinrVec; & \ac{SINR} vector \\
\\
$\UCP$ & \verb;\UCP; & Index of a given \ac{UCP} \\
$\UCPcons$ & \verb;\UCPcons; & Considered \ac{UCP} \\
$\AllUCP$ & \verb;\AllUCP; & Set of all possible \ac{UCP} \\
$\Code$ & \verb;\Code; & Code selected \\
$\CollClus$ & \verb;\CollClus; & Collision Cluster \\
\hline \hline
\end{tabular}
\end{center}


\begin{center}
\begin{tabular}{ l l l}
\hline \hline
$\RStart$ & \verb;\RStart; & Start time of a replica \\
$\VL$ & \verb;\VL; & Left shift w.r.t. to the replica start where the Vulnerable period starts \\
$\VR$ & \verb;\VR; & Right shift w.r.t. to the replica start where the Vulnerable period ends \\
$\Vg$ & \verb;\Vg; & For the asynchronous protocols, symmetric time shift \\
$\Vpd$ & \verb;\Vpd; & Vulnerable period duration \\
$\nVp$ & \verb;\nVp; & Number of vulnerable periods per \ac{VF} \\
\\
$\mU$ & \verb;\mU; & Number of possible selections of 2 users out of m \\
$\sL$ & \verb;\sL; & Number of ways to select slots in $\UCPcons$ \\
$\UL$ & \verb;\UL; & Number of ways to select slots in $\UCPcons$ for two users \\
\\
$\intFreeAsy$ & \verb;\intFreeAsy; & Fraction of interference free replica for async. RA \\
$\intFreeMRC$ & \verb;\intFreeMRC; & Fraction of interference free replica for RA after MRC \\
$\intOne$ & \verb;\intOne; & Portion of combined observation interfered only in one portion  \\
$\rateFree$ & \verb;\rateFree; & Rate corresponding to the interference free part of the replica \\
$\rateInt$ & \verb;\rateInt; & Rate corresponding to the interfered part of the replica \\
$\rateIntO$ & \verb;\rateIntO; & Rate corresponding to the interfered part of the replica \\
$\rateIntT$ & \verb;\rateIntT; & Rate corresponding to the interfered part of the replica \\
\\
\hline \hline
\end{tabular}
\end{center}







\clearpage 

==> chapter4/sections/notation.tex <==
\newtheorem{thm}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{coroll}{Corollary}
\newtheorem{prop}{Proposition}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}

\newcommand{\load}{\mathsf{G}}
\newcommand{\tp}{\mathsf{S}}
\newcommand{\se}{\xi}
\newcommand{\plr}{\mathsf{p}_l}
\newcommand{\rate}{\mathsf{R}}
\newcommand{\maxRate}{\mathsf{R}^*}
\newcommand{\mutInf}{\mathsf{I}}
\newcommand{\rvDec}{\mathcal{D}}

\newcommand{\capacity}{\mathsf{C}}
\newcommand{\capacitySC}{\capacity_\mathrm{S}}
\newcommand{\capacityMRC}{\capacity_\mathrm{M}}
\newcommand{\refCap}{\mathsf{C}_g}
\newcommand{\maxCap}{\mathsf{C}^*}
\newcommand{\maxSe}{\se^*}
\newcommand{\normCap}{\eta}

\newcommand{\dg}{\mathsf{d}}

\newcommand{\fraLen}{T_f}
\newcommand{\pkLen}{T_p}
\newcommand{\symLen}{T_s}
\newcommand{\fraTp}{n_p}
\newcommand{\VFStart}{T}
\newcommand{\RefTime}{t_0}
\newcommand{\Wind}{W}
\newcommand{\WindSh}{\Delta \Wind}

\newcommand{\numUs}{n_u}
\newcommand{\numSym}{n_s}
\newcommand{\numBit}{k}

\newcommand{\rx}{y}
\newcommand{\rxVec}{\bm{\rx}}
\newcommand{\tx}{x}
\newcommand{\txVec}{\bm{\tx}}
\newcommand{\noise}{n}
\newcommand{\noisePr}{\nu}
\newcommand{\noiseVec}{\bm{\noise}}
\newcommand{\noiseVar}{\sigma_{\noise}^2}
\newcommand{\intVal}{z}
\newcommand{\intVec}{\bm{\intVal}}
\newcommand{\intNum}{m}
\newcommand{\ch}{h}
\newcommand{\symVal}{a}
\newcommand{\pulse}{g}
\newcommand{\pulseRoot}{h}

\newcommand{\tm}{t}
\newcommand{\epoch}{\epsilon}
\newcommand{\freq}{f}
\newcommand{\phase}{\varphi}

\newcommand{\user}{u}
\newcommand{\replica}{r}
\newcommand{\sym}{s}

\newcommand{\usPw}{\mathsf{P}}
\newcommand{\PwAg}{\usPw_g}
\newcommand{\usPwTx}{\usPw_t}
\newcommand{\noisePw}{\mathsf{N}}
\newcommand{\noiseSD}{N_0}
\newcommand{\intPw}{\mathsf{Z}}
\newcommand{\sinr}{\gamma}
\newcommand{\sinrVec}{\Gamma}

\newcommand{\UCP}{\mathcal{L}}
\newcommand{\UCPcons}{\mathcal{L}^*}
\newcommand{\AllUCP}{\mathcal{L}_\mathrm{S}}
\newcommand{\Code}{\mathcal{C}}
\newcommand{\CollClus}{\mathcal{S}}

\newcommand{\RStart}{\tau}
\newcommand{\VL}{\RStart_l^*}
\newcommand{\VR}{\RStart_r^*}
\newcommand{\Vg}{\RStart^*}
\newcommand{\Vpd}{T_v}
\newcommand{\nVp}{n_v}

\newcommand{\mU}{\alpha_u}
\newcommand{\sL}{\beta_d}
\newcommand{\UL}{\beta_{u-d}}

\newcommand{\intFreeAsy}{\varphi_a}
\newcommand{\intFreeMRC}{\varphi_m}
\newcommand{\intOne}{\mu}
\newcommand{\rateFree}{\rate_f}
\newcommand{\rateInt}{\rate_i}
\newcommand{\rateIntO}{\rate_{i1}}
\newcommand{\rateIntT}{\rate_{i2}}

%%%%% Color for Editorial Changes
\definecolor{gl}{rgb}{0.0,0.5,0.8}
\definecolor{fc}{rgb}{0.8,0.5,0}
\definecolor{al}{rgb}{1,0.3,0.3}
\newcommand{\giangio}{\textcolor{gl}}
\newcommand{\fede}{\textcolor{fc}}
\newcommand{\alert}{\textcolor{al}}








==> chapter4/sections/preamble.tex <==
\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}

\newcommand{\fede}[1]{\textcolor{red}{#1}}
\newcommand{\giangio}{\textcolor{blue!80}}
\newcommand{\andrea}{\textcolor{green!80}}

%%%% Notation

\newcommand{\ET}{\mathrm{E}_T}    %% Tx energy
\newcommand{\EL}{\mathrm{E}_L}    %% Listen energy
\newcommand{\EI}{\mathrm{E}_I}    %% Idle energy
\newcommand{\E}{\mathrm{E}}		  % % Total average energy


\newcommand{\La}{\Lambda}    %% Node oriented dd (user)
\newcommand{\Rh}{\mathrm{P}}    %% Node oriented dd (slot)
\newcommand{\la}{\lambda}    %% edge oriented dd (user)
\newcommand{\rh}{\rho}    %% egde oriented dd (slot)

\newcommand{\iLa}[1]{\Lambda^{(#1)}}    %% Induced Node oriented dd (user)
\newcommand{\iRh}[1]{\mathrm{P}^{(#1)}}    %% Induced  Node oriented dd (slot)
\newcommand{\ila}[1]{\lambda^{(#1)}}    %% Induced edge oriented dd (user)
\newcommand{\irh}[1]{\rho^{(#1)}}    %% Induced  egde oriented dd (slot)

\newcommand{\graph}{\mathscr{G}}    %% Graph
\newcommand{\uset}{\mathscr{U}}    %% user nodes set
\newcommand{\sset}{\mathscr{S}}    %% slot nodes set
\newcommand{\listset}{\mathscr{L}}    %% listen set
\newcommand{\sn}{\mathsf{s}}    %% listen set
\newcommand{\un}{\mathsf{u}}    %% listen set


\newcommand{\dum}{\mathtt{x}}    %% dummy variable

\newcommand{\load}{\mathsf{G}}    %% channel load
\newcommand{\thrp}{\mathsf{R}_{\mathrm{D}}}    %% throughput
\newcommand{\plr}{\mathsf{P}_{\mathrm{MD}}}    %% PLR

\newcommand{\thr}{\mathsf{G}^\star}    %% threshold
\newcommand{\plrt}{\plr^\star}    %% PLR

\newcommand{\slots}{n} % % number of slots per discovery phase
\newcommand{\tslot}{\mathrm{T}_s} % % number of slots per discovery phase
\newcommand{\users}{m} % % number of users in the network

\newcommand{\degree}{d} % % number of replicas sent per user, i.e. degree
\newcommand{\listn}{\ell} % % listening probability
\newcommand{\dmax}{{\degree_{\mathrm{max}}}}    %% Node oriented dd (user)
\newcommand{\avgd}{\bar\degree}    %% Node oriented dd (user)

\newcommand{\dcost}{\mathrm{D}_C}    %% Node oriented dd (user)


\newcommand\T{\rule{0pt}{2.6ex}}


==> chapter6/sections/ack.tex <==
\section*{Acknowledgment}\label{sec:ack}

The authors would like to thank Dr. Gianluigi Liva (German Aerospace Center) and Prof. Marco Chiani (University of Bologna) for fruitful discussions. 

==> chapter6/sections/title.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%

 % !TEX root =  ../GC_CSA_Fading_6.0.tex

%\title{Asymptotic Analysis of Coded Slotted Aloha on the Rayleigh Block Fading Channel}
\title{Irregular Repetition Slotted ALOHA over the Rayleigh Block Fading Channel with Capture}
%\author{
%Iacopo Mambelli, Federico Clazzer, Gianluigi Liva, Enrico Paolini and Marco Chiani
%\thanks{Iacopo Mambelli, Enrico Paolini and Marco Chiani are with CNIT, DEI, University of Bologna,
%via Venezia 52, 47521 Cesena (FC), Italy. E-mail: \texttt{\{e.paolini,marco.chiani\}@unibo.it}}
%\thanks{Federico Clazzer and Gianluigi Liva are with the Institute of Communications and
%Navigation of the German Aerospace Center (DLR), Muenchner Strasse 20, 82234
%Wessling, Germany.
%Email:\{\texttt{Federico.Clazzer}, \texttt{Gianluigi.Liva}\}\texttt{@dlr.de}.}}


\author{
    \IEEEauthorblockN{Federico Clazzer\IEEEauthorrefmark{1}, Enrico Paolini\IEEEauthorrefmark{2}, Iacopo Mambelli\IEEEauthorrefmark{3}, {\v C}edomir Stefanovi{\'c}\IEEEauthorrefmark{4}}\\
    \IEEEauthorblockA{\IEEEauthorrefmark{1}Institute of Communications and Navigation of DLR (German Aerospace Center),
    Wessling, Germany.}\\ %\\ Email: Federico.Clazzer@dlr.de}\\
    \IEEEauthorblockA{\IEEEauthorrefmark{2}Department of Electrical, Electronic, and Information Engineering, University of Bologna, Cesena, Italy.}\\%\\ Email: e.paolini@unibo.it}\\
    \IEEEauthorblockA{\IEEEauthorrefmark{3}Fores Engineering S.R.L., Forl{\`i}, Italy.}\\ %Email: iacopo.mambelli@fores.it}\\
    \IEEEauthorblockA{\IEEEauthorrefmark{4} Department of Electronic Systems, Aalborg University, Aalborg, Denmark.}% Email: cs@es.aau.dk}
}



 \maketitle
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%

\thispagestyle{empty}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{abstract}
Random access protocols relying on the transmission of packet replicas in multiple slots and exploiting interference cancellation at the receiver have been shown to achieve performance competitive with that of orthogonal schemes.
%The use of a variable number of copies for each transmitted packet leads to noticeable improvements w.r.t. \ac{SA}.
So far the optimization of the repetition degree profile, defining the probability for a user to transmit a given number of replicas, has mainly been performed targeting the collision channel model. In this paper the analysis is extended to a block fading channel model, also assuming capture effect at the receiver. Density evolution equations are developed for the new setting and, based on them, some repetition degree profiles are optimized and analyzed via Monte Carlo simulation in a finite frame length setting. The derived distributions are shown to achieve throughputs largely exceeding $\mathbf{1}$ $\mathrm{\mathbf{[packet/slot]}}$.
\end{abstract}


% The paper headers
%\markboth{submitted to IEEE Transactions on Communications}{F. Clazzer et al.: Asymptotic Analysis of Coded Slotted Aloha on the Rayleigh Block Fading Channel} %
% make the title area
% Don't write page number 0 to the cover page.

\thispagestyle{empty}
\setcounter{page}{1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\begin{keywords}
%\todo{To be written}
%\end{keywords}
%\pagenumbering{arabic}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> chapter7/tex/displaynotation.tex <==

\cleardoublepage

\section*{Notation}


%\bigskip

\begin{center}
\begin{tabular}{ l l l}
\hline \hline
$\load$ & \verb;\load; & Load \\
$\loadMax$ & \verb;\loadMax; & Load corresponding to the maximum throughput \\
$\tp$ & \verb;\tp; & Throughput \\
$\tpMax$ & \verb;\tpMax; & Maximum throughput \\
$\tpSA$ & \verb;\tpSA; & Throughput Slotted Aloha\\
$\tpUL$ & \verb;\tpUL; & Throughput Uplink\\
$\tpULMax$ & \verb;\tpULMax; & Maximum Throughput Uplink\\
$\tpULk{k}$ & \verb;\tpULk{k}; & Throughput Uplink with $k$ receivers\\
$\tpULkMax{k}$ & \verb;\tpULkMax{k}; & Maximum throughput uplink with $k$ receivers\\
$\tpDL$ & \verb;\tpDL; & Throughput Downlink\\
$\tpetoe$ & \verb;\tpetoe; & End-to-end throughput\\
$\ulrk{k}$ & \verb;\ulr; & User Loss Probability, i.e. probability that a packet is not received\\  & & by any of the $k$ relays\\
$\dlrate$ & \verb;\dlrate; & Downlink Rate\\
$\dlratek$ & \verb;\dlratek; & Downlink Rate to relay $k$\\
$\fracratek$ & \verb;\fracratek; & Downlink Rate\\
$\plos$ & \verb;\plos; & Burst loss probability (after decoding)\\
$\x$ & \verb;\x; & x as dummy variable\\
$\nrx$ & \verb;\nrx; & number of relays\\
$\rx$ & \verb;\rx; & considered relay\\
$\usersRV$ & \verb;\usersRV; & r.v. describing number of nodes accessing uplink slot\\
$\users$ & \verb;\users; &  number of nodes accessing uplink slot\\
$\peras$ & \verb;\peras; &  uplink packet erasure probability\\
$\collRV$ & \verb;\collRV; & r.v. describing number of collected packets\\
$\coll$ & \verb;\coll; &  number of collected packets\\
$\collMax$ & \verb;\collMax; &  Maximum number of collected packets\\
$\collK{k}$ & \verb;\collK{k}; &  number of collected packets at relay $k$\\
$\colVec$ & \verb;\colVec; &  vector of collected packets\\
$\colVecK{k}$ & \verb;\colVecK{k}; &  vector of collected packets at relay $k$\\
$\colNumVec$ & \verb;\colNumVec; &  vector of number of collected packets\\
\hline \hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{ l l l}
\hline \hline
$\linll$ & \verb;\linll; &  number of linear combination generated a generic relay\\
$\linllK{k}$ & \verb;\linllK{k}; &  number of linear combination generated by the $k$-th relay\\
$\linComb$ & \verb;\linComb; &  vector of linear combinations of packets generated\\
$\linCombK{k}$ & \verb;\linCombK{k}; &  vector of linear combinations of packets generated at relay $k$\\
$\MxComb$ & \verb;\MxComb; &  Matrix with coefficients for the linear combination of packets sent \\
& & from the relay to the gateway\\
$\MxCombK{k}$ & \verb;\MxComb{k}; &  Matrix with coefficients for the linear combination of packets sent \\
& & from the relay to the gateway subscript k\\
$\fieldOrd$ & \verb;\fieldOrd; & Gaolois field order of the linear comb. coefficients\\
$\capDL$ & \verb;\capDL; &  downlink capacity\\
$\ulslot$ & \verb;\ulslot; &  duration of uplink slot\\
$\dlslot$ & \verb;\dlslot; &  duration of downlink slot\\
$\numulslot$ & \verb;\numulslot; &  number of observed uplink slots\\
$\numdlslot$ & \verb;\numdlslot; &  number of employed downlink slots (for NC transmissions)\\
$\slot$ & \verb;\slot; &  generic slot\\
$\del$ & \verb;\del; &  delay\\
$\maxdel$ & \verb;\maxdel; &  maximum delay\\
$\bufsize$ & \verb;\bufsize; &  buffer size\\
$\mxNumRow$ & \verb;\mxNumRow; &  Row Number in Matrix\\
$\mxNumCol$ & \verb;\mxNumCol; &  Column Number in Matrix\\
$\elOne$ & \verb;\elOne; & Generic coefficient element in the Matrix $\MxComb$\\
$\elOneK{1,1}$ & \verb;\elOneK{1,1}; & Specific Coefficient element in the Matrix $\MxComb$\\
$\elTwo$ & \verb;\elTwo; & Generic coefficient element in the Matrix $\MxComb$\\
$\elTwoK{1,1}$ & \verb;\elTwoK{1,1}; & Specific Coefficient element in the Matrix $\MxComb$\\
$\rank$ & \verb;\rank; & Matrix rank\\
$\rankK{k}$ & \verb;\rankK{k}; & Matrix rank of submatrix $k$\\
$\rankKMax{k}$ & \verb;\rankKMax{k}; & Maximum matrix rank of submatrix $k$\\
$\rankNumVec$ & \verb;\rankNumVec; &  vector of rank values\\
$\mxCol$ & \verb;\mxCol; & Matrix col number\\
$\mxColK{k}$ & \verb;\mxColK{k}; & Matrix col number of submatrix $k$\\
\hline \hline
\end{tabular}
\end{center}











\clearpage 

==> chapter7/tex/notation.tex <==
\newtheorem{thm}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{coroll}{Corollary}
\newtheorem{prop}{Proposition}
\newtheorem{result}{Result}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}


\newcommand{\ul}{ul}
\newcommand{\dl}{dl}
\newcommand{\load}{\mathsf{G}}
\newcommand{\loadMax}{\load^{*}}
\newcommand{\tp}{\mathsf{S}}
\newcommand{\tpMax}{\tp^{*}}
\newcommand{\tpSA}{\tp_{sa}}
\newcommand{\tpUL}{\tp_{\ul}}
\newcommand{\tpULMax}{\tpMax_{\ul}}
\newcommand{\tpULk}[1]{\tp_{\ul,#1}}
\newcommand{\tpULkMax}[1]{\tpMax_{\ul,#1}}
\newcommand{\tpDL}{\tp_{\dl}}
\newcommand{\tpetoe}{\tp_{e2e}}
\newcommand{\ulrk}[1]{\zeta_{#1}}
\newcommand{\dlrate}{\mathsf{R}}
\newcommand{\dlratek}{\mathsf{R}_k}
\newcommand{\fracratek}{z_k}
\newcommand{\plos}{\xi}
\newcommand{\x}{\mathtt{x}}
\newcommand{\qtarget}{\bar{\mathtt{q}}}
\newcommand{\plostarget}{\bar{\plos}}
\newcommand{\nrx}{K}
\newcommand{\rx}{k}
\newcommand{\usersRV}{U}
\newcommand{\users}{u}
\newcommand{\collRV}{C}
\newcommand{\coll}{c}
\newcommand{\collMax}{\coll^{*}}
\newcommand{\collK}[1]{\coll_{#1}}
\newcommand{\colVec}{\ve c}
\newcommand{\colVecK}[1]{\colVec_{#1}}
\newcommand{\linll}{r}
\newcommand{\linllK}[1]{\linll_{#1}}
\newcommand{\linComb}{\ve \linll}
\newcommand{\linCombK}[1]{\linComb_{#1}}
\newcommand{\MxComb}{\ve M}
\newcommand{\MxCombK}[1]{\MxComb_{#1}}
\newcommand{\fieldOrd}{q}
\newcommand{\peras}{\varepsilon}
\newcommand{\capDL}{\mathsf{C_{\dl}}}
\newcommand{\ulslot}{\mathsf{T_{\ul}}}
\newcommand{\dlslot}{\mathsf{T_{\dl}}}
\newcommand{\numulslot}{m_{\ul}}
\newcommand{\numdlslot}{m_{\dl}}
\newcommand{\slot}{m}
\newcommand{\del}{\mathsf{D}}
\newcommand{\maxdel}{\mathsf{D}_{max}}
\newcommand{\bufsize}{B}
\newcommand{\mxNumRow}{a}
\newcommand{\mxNumCol}{b}
\newcommand{\elOne}{\alpha}
\newcommand{\elOneK}[1]{\elOne_{#1}}
\newcommand{\elTwo}{\beta}
\newcommand{\elTwoK}[1]{\elTwo_{#1}}
\newcommand{\rank}{n}
\newcommand{\rankK}[1]{\rank_{#1}}
\newcommand{\rankKMax}[1]{\rankK{#1}^{*}}
\newcommand{\mxCol}{h}
\newcommand{\mxColK}[1]{\mxCol_{#1}}
\newcommand{\colNumVec}{\ve{\hat{\coll}}}
\newcommand{\rankNumVec}{\ve{\hat{\rank}}}


\newcommand{\oleq}[1]{\overset{\text{(#1)}}{\leq}}
\newcommand{\oeq}[1]{\overset{\text{(#1)}}{=}}
\newcommand{\ogeq}[1]{\overset{\text{(#1)}}{\geq}}
\newcommand{\ogeql}[2]{\overset{#1}{\underset{#2}{\gtreqless}}}










%%%%% Color for Editorial Changes
\definecolor{gl}{rgb}{0.0,0.5,0.8}
\definecolor{fc}{rgb}{0.8,0.5,0}
\definecolor{al}{rgb}{1,0.3,0.3}
\newcommand{\giangio}{\textcolor{gl}}
\newcommand{\fede}{\textcolor{fc}}
\newcommand{\alert}{\textcolor{al}}








==> sections/acronyms.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% abbreviations.bib
%%%
%%% \acresetall resets all acronyms to not used. Useful after the abstract to redefine all acronyms in the introduction.
%%% \acf{label} Full: written out form with acronym in parentheses, irrespective of previous use
%%% \acs{label} acronym form, irrespective of previous use
%%% \acl{label} written out form without following acronym
%%% \acp{label} plural form of acronym by adding an s. \acfp. \acsp, \aclp work as well.
%%% \acs{label} Short: short version of the acronym
%%% \acfp, acsp aclp acfi acused acsu aclu
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{acronym}
% A
\acro{A/A}{air-to-air}%
\acro{A-EXEC}{auto execute COCR service}%
\acro{AAC}{airline administrative control}%
\acro{ACK}{acknowledgement}%
\acro{ACP}{aeronautical communications panel}%
\acro{AF}{assured forwarding}%
\acro{AL}{application layer}%
\acro{ANSP}{air navigation service provider}%
\acro{AOC}{airline operational control}%
\acro{APC}{air passenger communication}%
\acro{APT}{airport}%
\acro{ATC}{air traffic control}%
\acro{ATI}{access technology independent}%
\acro{ATM}{air traffic management}%
\acro{ATN}{aeronautical telecommunication network}%
\acro{ATN/IPS}{aeronautical telecommunication network / internet protocol suite}%
\acro{ATN/OSI}{aeronautical telecommunication network / open systems interconnection reference model}%
\acro{ATS}{air traffic services}%
\acro{ATSC}{air traffic service communication}%
\acro{AVBDC}{absolute volume based dynamic capacity}%
\acro{AWGN}{additive white gaussian noise}%
% B
\acro{BB}{bandwidth broking} %
\acro{BBFRAME}{baseband frame}%
\acro{BE}{best effort}%
\acro{BER}{bit error rate}%
\acro{BGAN}{broadband global area network}%
\acro{BSM}{broadband satellite multimedia}%
% C
\acro{CA}{constrained architecture}%
\acro{CAC}{connection admission Control}%
\acro{CC}{congestion control}%
\acro{CDF}{cumulative distribution function}
\acro{CDMA}{code divison multiple access}%
\acro{CLNP}{connectionless networking protocol}%
\acro{CLTP}{connectionless transport protocol}%
\acro{CoA}{care of address}%
\acro{CoS}{class of service}%
\acro{COCR}{communications operating concept and requirements for the future radio system}%
\acro{COTP}{connection oriented transport protocol}%
\acro{COTS}{commercial-off-the-shelf}%
%%\acro{CRA}{Constant Rate Assignment}%
\acro{CRA-CC}{CRA-convolutional code}%
\acro{CRA-SH}{CRA-shannon bound}%
\acro{CRA}{contention resolution ALOHA}%
\acro{CRC}{cyclic redundancy check}%
\acro{CRDSA}{contention resolution diversity slotted ALOHA}%
\acro{CRDSA++}{contention resolution diversity slotted ALOHA++}%
\acro{CS}{class selector}%
\acro{CSA}{coded slotted ALOHA}%
\acro{CSMA}{carrier sense multiple access}%
% D
\acro{DAMA}{demand assigned multiple access}%
\acro{DiffServ}{differentiated services}%
\acro{DoD}{department of defence}%
\acro{DSA}{diversity slotted ALOHA}%
\acro{DSCP}{diffServ code point}%
\acro{DVB}{digital video broadcasting}%
\acro{DVB-RCS+M}{digital video broadcasting - return channel via satellite mobility}%
\acro{DVB-RCS}{digital video broadcasting - return channel via satellite}%
\acro{DVB-S2}{digital video broadcasting - second generation}%
\acro{DVB-S2/RCS}{digital video broadcasting - second generation / return channel via satellite}%
% E
\acro{ECN}{explicite congestion notification}%
\acro{ECRA}{enhanced contention resolution ALOHA}%
\acro{ECRA-SC}{ECRA selection combining}
\acro{ECRA-MRC}{ECRA maximal ratio combining}
\acro{ECTL}{eurocontrol}%
\acro{EF}{expedited forwarding}%
\acro{EGD}{equal-gain diversity}
\acro{ENR}{en-route}%
\acro{ES}{end system}%
\acro{ESA}{European space agency}%
\acro{ETSI}{European telecommunications standards institute}%
\acro{ETSI-BSM}{European telecommunications standards institute - broadband satellite multimedia}%
% F
\acro{FAA}{federal aviation administration}%
\acro{FCA}{free capacity assignment}%
\acro{FDM}{frequency division multiplexing}%
\acro{FDMA}{frequency division multiple access}%
\acro{FEC}{forward error correction}%
\acro{FET}{first entry times}%
\acro{FL}{forward link}%
% G
\acro{GEO}{geostationary orbit}%
\acro{GIG}{global information grid}%
\acro{GSE}{generic stream encapsulation}%
% H
\acro{HA}{home agent}%
\acro{HF}{high frequency}%
% I
\acro{IC}{interference cancellation}%
\acro{ICAO}{international civil aviation organization}%
\acro{IETF}{internet engineering task force}%
\acro{IntServ}{integrated services}%
\acro{IP}{internet protocol}%
\acro{IPS}{internet protocol suite}%
\acro{IPSec}{IP security}%
\acro{IRCRA}{irregular repetition contention resolution ALOHA}%
\acro{IRSA}{irregular repetition slotted ALOHA} %
\acro{IS}{intermediate system}%
\acro{IS-IS-TE}{intermediate system to intermediate system extension for traffic engineering}%
\acro{ISI}{input stream identifier}%
\acro{ISO/OSI}{international organization for standardization/open systems interconnection}%
% K
\acro{Ku}{kurz-under}%
\acro{Ka}{kurz-above}%
% L
\acro{LAE}{link access equipment}%
\acro{LAN}{local area network}%
\acro{LD}{low density}%
\acro{LDACS}{L-band digital aeronautical communication system}%
\acro{L-DACS}{L-band digital aeronautical communication system}%
\acro{LDPC}{low density parity check codes}%
\acro{LEO}{low earth orbit}%
% M
\acro{M2M}{machine-to-machine}
\acro{MAC}{medium access}%
\acro{MCAST}{multicast}%
\acro{MF-TDMA}{multifrequency time division multiple access}%
\acro{MH}{mobile host}%
\acro{MIHF}{Media independent handover function}%
\acro{MLPP}{multi level priority preemption}%
\acro{Mode-S}{mode-select}%
\acro{MPE}{multi protocol encapsulation}%
\acro{MPEG2-TS}{MPEG2 - transport stream}%
\acro{MPLS}{multi protocol label switching}%
\acro{MRC}{maximal-ratio combining}
% N
\acro{NCC}{network control centre}%
\acro{NET}{network connectivity}
\acro{NEWSKY}{NEtWorking the SKY for aeronautical communications}%
\acro{NOC}{non-operational communication}%
\acro{NSIS}{next steps in signalling}%
% O
\acro{OC}{operational communication}%
\acro{ORP}{oceanic, remote and polar}%
\acro{OSI}{open systems interconnection}%
\acro{OSPF}{open shortes path first}%
% P
\acro{PDF}{probability density function}%
\acro{PCE}{predictive capacity estimation}%
\acro{PCN}{pre-congestion notification}%
\acro{PDU}{protocol data unit}%
\acro{PEP}{performance enhancing proxy}%
\acro{PER}{packet error rate}%
\acro{PID}{packet identifier}%
\acro{PLFRAME}{physical layer frame}%
\acro{PLR}{packet loss rates}%
% Q
\acro{QoS}{quality of service}%
\acro{QoS-PRN}{QoS private relay nodes}%
\acro{QoS-RN}{QoS-relay nodes}%
% R
\acro{RA}{random access}%
\acro{RBDC}{rate based dynamic capacity}%
\acro{RCB}{random coding bound}%
\acro{RCS}{return channel via satellite}%
\acro{RCS+M}{return channel via satellite plus mobility}%
\acro{RF}{radio frequency}%
\acro{RFC}{request for comments}%
\acro{RL}{return link}%
\acro{RM}{resource management}%
\acro{RN}{relay nodes}%
\acro{RRM}{radio resource management}%
\acro{RS}{reed solomon}%
\acro{RSVP}{resource reservation protocol}%
\acro{RTT}{round trip time}%
% S
\acro{SA}{slotted ALOHA}%
\acro{SANDRA}{seamless aeronautical networking through integration of data links, radios and antennas}%
\acro{SB}{Shannon bound}%
\acro{S2}{second generation}%
\acro{SC}{selection combining}
\acro{SESAR}{single European sky ATM research}%
\acro{SF}{superframe}%
\acro{SIC}{successive interference cancellation}%
\acro{SLS}{service level specification}%
\acro{SNDCF}{subnetwork dependent convergence function}%
\acro{SNIR}{signal-to-noise and interference ratio}%
\acro{SNR}{signal-to-noise ratio}%
\acro{SWIM}{system wide information management}%
\acro{SYN}{synchronization}%
\acro{SYNC}{synchronization}%
% T
\acro{TCP}{transport control protocol}%
\acro{TCP/IP}{transport control protocol / internet protocol suite}%
\acro{TDMA}{time division multiple access}%
\acro{TE}{traffic engineering}%
\acro{TI}{technology independent}%
\acro{TI-SAP}{technology independent - service access point}%
\acro{TD}{technology dependent}%
\acro{TL}{transport layer}%
\acro{TMA}{terminal maneuvering area}%
\acro{ToS}{type of service}%
% U
\acro{UCA}{unconstrained architecture}%
\acro{UDP}{user datagram protocol}%
% V
\acro{VBDC}{volume based dynamic capacity}%
\acro{VDL}{VHF digital mode}%
\acro{VHF}{very high frequency}%
\acro{VoIP}{voice over IP}%
\acro{VPN}{virtual private networks}%
% W
\acro{WG}{working group}%
\acro{WiMAX}{worldwide interoperability for microwave access}%
% X
\acro{XFECFRAME}{forward error correction frame}%
\end{acronym}

\makeatletter
\newif\ifAC@uppercase@first
\def\Aclp#1{\AC@uppercase@firsttrue\aclp{#1}\AC@uppercase@firstfalse}
\def\AC@aclp#1{%
  \ifcsname fn@#1@PL\endcsname
    \ifAC@uppercase@first
      \expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname
    \else
      \csname fn@#1@PL\endcsname
    \fi
  \else
    \AC@acl{#1}s
  \fi 
}
\edef\AC@uppercase@write{\string\ifAC@uppercase@first\string\expandafter\string\MakeUppercase\string\fi\space}
\def\AC@acrodef#1[#2]#3{%
  \@bsphack
  \protected@write\@auxout{}{%
    \string\newacro{#1}[#2]{\AC@uppercase@write #3}%
  }\@esphack
}
\def\Acl#1{\AC@uppercase@firsttrue\acl{#1}\AC@uppercase@firstfalse}
\makeatother


==> sections/displaynotation.tex <==

\cleardoublepage

\section*{Notation}


\bigskip

\begin{center}
\begin{tabular}{ l l l}
\hline \hline
$\load$ & \verb;\load; & Load \\
$\tp$ & \verb;\tp; & Throughput \\
$\tpLT$ & \verb;\tpLT; & Layer $3$ Throughput \\
$\se$ & \verb;\se; & Spectral Efficiency \\
$\plr$ & \verb;\plr; & Packet Loss Rate \\
$\plrLT$ & \verb;\plrLT; & Layer $3$ Packet Loss Rate \\
$\psucc$ & \verb;\psucc; & Packet Successful Probability \\
$\psuccLT$ & \verb;\psuccLT; & Packet Successful Probability Layer $3$ packets\\
$\psuccLTAppr$ & \verb;\psuccLTAppr; & Approximation Packet Successful Probability Layer $3$ packets\\
$\rate$ & \verb;\rate; & Rate \\
$\maxRate$ & \verb;\maxRate; & Maximum Rate allowed\\
$\mutInf$ & \verb;\mutInf; & Mutual information\\
$\rvDec$ & \verb;\rvDec; & r.v. denoting the outcome of the decoding process\\
$\capacity$ & \verb;\capacity; & Capacity \\
$\capacitySC$ & \verb;\capacitySC; & Capacity selection combinig\\
$\capacityMRC$ & \verb;\capacityMRC; & Capacity maximal-ratio combining\\
$\refCap$ & \verb;\refCap; & Reference Capacity of the Gaussian MAC \\
$\maxCap$ & \verb;\maxCap; & Maximum Capacity \\
$\maxSe$ & \verb;\maxSe; & Maximum spectral efficiency \\
$\normCap$ & \verb;\normCap; & Normalized capacity \\
\\
$\dg$ & \verb;\dg; & Number of replicas per user, i.e. degree \\
$\ratethr$ & \verb;\ratethr; & Rate threshold \\
$\snrthr$ & \verb;\snrthr; & \ac{SNR} threshold \\
\hline \hline
\end{tabular}
\end{center}


\begin{center}
\begin{tabular}{ l l l}
\hline \hline
$\fraLen$ & \verb;\fraLen; & VF duration \\
$\pkLen$ & \verb;\pkLen; & Packet duration \\
$\symLen$ & \verb;\symLen; & Symbol duration \\
$\slLen$ & \verb;\slLen; & Slot duration \\
$\fraTp$ & \verb;\fraTp; & Duration of VF in packets durations \\
$\VFStart$ & \verb;\VFStart; & Delay w.r.t. the VF start \\
$\RefTime$ & \verb;\RefTime; & User delay w.r.t. the common reference time \\
$\Wind$ & \verb;\Wind; & Decoder window size \\
$\WindSh$ & \verb;\WindSh; & Decoder window shift \\
\\
$\numUs$ & \verb;\numUs; & number of user/transmission terminals \\
$\numUsB$ & \verb;\numUsB; & number of backlogged user (Chapter 1) \\
$\numSym$ & \verb;\numSym; & number of symbols in a packet/replica \\
$\sw$ & \verb;\sw; & Subscript for sync word\\
$\syncSym$ & \verb;\syncSym; & Number of sync word symbols\\
$\numSlot$ & \verb;\numSlot; & number of slot in a frame \\
$\numBit$ & \verb;\numBit; & number of information bits per packet/replica \\
\\
$\rx$ & \verb;\rx; & received signal \\
$\rxTwo$ & \verb;\rxTwo; & received signal modified\\
$\rxVec$ & \verb;\rxVec; & vector of received samples/symbols \\
$\rxrv$ & \verb;\rxrv; & r.v. received signal \\
$\rxrvVec$ & \verb;\rxrvVec; & vector of r.v. received signal \\
$\tx$ & \verb;\tx; & transmitted signal \\
$\txVec$ & \verb;\txVec; & vector of transmitted samples/symbols \\
$\noise$ & \verb;\noise; & noise signal \\
$\noisePr$ & \verb;\noisePr; & white Gaussian process \\
$\noiseVec$ & \verb;\noiseVec; & vector of noise samples \\
$\noiseVar$ & \verb;\noiseVar; & noise variance \\
$\intVal$ & \verb;\intVal; & interference random variable \\
$\intVec$ & \verb;\intVec; & vector of interference samples \\
$\intVar$ & \verb;\intVar; & interference variance \\
$\noiseInt$ & \verb;\noiseInt; & noise and interference contribution \\
$\intNum$ & \verb;\intNum; & number of interferers \\
$\intRV$ & \verb;\intRV; & r.v. representing the number of interferers \\
$\symVal$ & \verb;\symVal; & value of the transmitted symbol \\
$\pulse$ & \verb;\pulse; & pulse shape raised cosine filter \\
$\pulseRoot$ & \verb;\pulseRoot; & pulse shape root raised cosine filter \\
\hline \hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{ l l l}
\hline \hline
$\tm$ & \verb;\tm; & time \\
$\epoch$ & \verb;\epoch; & epoch \\
$\freq$ & \verb;\freq; & frequency \\
$\phase$ & \verb;\phase; & phase \\
\\
$\user$ & \verb;\user; & user index \\
$\replica$ & \verb;\replica; & replica index \\
$\sym$ & \verb;\sym; & Symbol\\
$\symVec$ & \verb;\symVec; & Vector of symbols\\
\\
$\reTx$ & \verb;\reTx; & Retransmission dummy r.v. Chapter 1 \\
\\
$\usPw$ & \verb;\usPw; & useful received power \\
$\PwAvg$ & \verb;\PwAvg; & average received power \\
$\PwAg$ & \verb;\PwAg; & Aggregated recevied power \\
$\usPwTx$ & \verb;\usPwTx; & User transmission power \\
$\noisePw$ & \verb;\noisePw; & noise power \\
$\noiseSD$ & \verb;\noiseSD; & single-sided noise power spectral density \\
$\EnSym$ & \verb;\EnSym; & Energy per symbol \\
$\intPw$ & \verb;\intPw; & interference power \\
$\intPwVec$ & \verb;\intPwVec; & interference power vector \\
$\sinr$ & \verb;\sinr; & \ac{SINR} \\
$\sinrVec$ & \verb;\sinrVec; & \ac{SINR} vector \\
\\
$\UCP$ & \verb;\UCP; & Index of a given \ac{UCP} \\
$\UCPcons$ & \verb;\UCPcons; & Considered \ac{UCP} \\
$\AllUCP$ & \verb;\AllUCP; & Set of all possible \ac{UCP} \\
$\Code$ & \verb;\Code; & Code selected \\
$\CollClus$ & \verb;\CollClus; & Collision Cluster \\
\hline \hline
\end{tabular}
\end{center}


\begin{center}
\begin{tabular}{ l l l}
\hline \hline
$\RStart$ & \verb;\RStart; & Start time of a replica \\
$\VL$ & \verb;\VL; & Left shift w.r.t. to the replica start where the Vulnerable period starts \\
$\VR$ & \verb;\VR; & Right shift w.r.t. to the replica start where the Vulnerable period ends \\
$\Vg$ & \verb;\Vg; & For the asynchronous protocols, symmetric time shift \\
$\Vpd$ & \verb;\Vpd; & Vulnerable period duration \\
$\nVp$ & \verb;\nVp; & Number of vulnerable periods per \ac{VF} \\
\\
$\mU$ & \verb;\mU; & Number of possible selections of 2 users out of m \\
$\sL$ & \verb;\sL; & Number of ways to select slots in $\UCPcons$ \\
$\UL$ & \verb;\UL; & Number of ways to select slots in $\UCPcons$ for two users \\
\\
$\intFreeAsy$ & \verb;\intFreeAsy; & Fraction of interference free replica for async. RA \\
$\intFreeMRC$ & \verb;\intFreeMRC; & Fraction of interference free replica for RA after MRC \\
$\intOne$ & \verb;\intOne; & Portion of combined packet interfered only in one portion  \\
$\rateFree$ & \verb;\rateFree; & Rate corresponding to the interference free part of the replica \\
$\rateInt$ & \verb;\rateInt; & Rate corresponding to the interfered part of the replica \\
$\rateIntO$ & \verb;\rateIntO; & Rate corresponding to the interfered part of the replica \\
$\rateIntT$ & \verb;\rateIntT; & Rate corresponding to the interfered part of the replica \\
\\
$\off$ & \verb;\off; & Time Offset \\
$\arrRate$ & \verb;\arrRate; & Total arrival rate for Poisson arrivals in ALOHA \\
& & (Chapter 1) and SICTA (Chapter 3)\\
$\maxWinSize$ & \verb;\maxWinSize; & Maximum window size in windowed access \\
& & for tree-splitting algorithms \\
$\finWin$ & \verb;\finWin; & Time interval elapsed from the end of the current window \\
& & to the end of the \ac{CRI} \\
$\prob$ & \verb;\prob; & Generic probability. Used in the SICTA algorithm description.\\
$\CRIL$ & \verb;\CRIL; & CRI lenght. Used in the SICTA algorithm description\\
$\cntL$ & \verb;\cntL; & Local counter. Used in the SICTA algorithm description\\
$\cntS$ & \verb;\cntS; & System counter. Used in the SICTA algorithm description\\
$\tsd$ & \verb;\tsd; & Splitting factor. Used in the SICTA algorithm description\\
\\
$\mx$ & \verb;\mx; & Generic Matrix.\\
$\vc$ & \verb;\vc; & Generic Vector.\\
\hline \hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{ l l l}
\hline \hline
$\bs$ & \verb;\bs; & Binary sequence. Used for the chapter on \\
& & \ac{RA} without feedback\\
$\bse$ & \verb;\bse; & Binary sequence element. Used for the chapter on \ac{RA} \\
& & without feedback\\
$\lbs$ & \verb;\lbs; & Binary sequence length. Used for the chapter on \ac{RA} \\
& & without feedback\\
$\ts$ & \verb;\ts; & Time shift. Used for the chapter on \ac{RA} without feedback\\
$\df$ & \verb;\df; & Protocol sequence duty factor. Used for the chapter on \ac{RA}\\
 & & without feedback\\
\\
$\TestThrOne$ & \verb;\TestThrOne; & Non-coherent soft-correlation test\\
$\TestThrTwo$ & \verb;\TestThrTwo; & Non-coherent soft-correlation test entire packet\\
$\TestThrInt$ & \verb;\TestThrInt; & Non-coherent soft-correlation test \\
& & with interference\\
$\ThrCorr$ & \verb;\ThrCorr; & Threshold for the non-coherent soft-correlation test\\
$\ThrCorrInt$ & \verb;\ThrCorrInt; & Threshold for the non-coherent soft-correlation \\
& & test modified\\
$\HypAbove$ & \verb;\HypAbove; & Hypothesis of having a packet\\
$\HypBelow$ & \verb;\HypBelow; & Hypothesis of only noise\\
$\Hyp$ & \verb;\Hyp; & Generic Hypothesis\\
$\DecAbove$ & \verb;\DecAbove; & Decision of having a packet\\
$\DecBelow$ & \verb;\DecBelow; & Decision of only noise\\
$\RStartSet$ & \verb;\RStartSet; & Set of replicas starting positions\\
$\SlotSize$ & \verb;\SlotSize; & Slot dimension in the async. slotted case for ECRA\\
$\nSlotsSmall$ & \verb;\nSlotsSmall; & Number of small slots\\
$\probFalse$ & \verb;\probFalse; & False Alarm probability\\
$\probDet$ & \verb;\probDet; & Detection probability\\
$\probCorComb$ & \verb;\probCorComb; & Correct combining probability\\
\\
$\LDist$ & \verb;\LDist; & Probability measure defining the packet length distribution\\
$\LDistDisc$ & \verb;\LDistDisc; & Probability measure defining the packet length distribution discretized\\
$\FragO$ & \verb;\FragO; & Fragmentation overhead\\
$\PadO$ & \verb;\PadO; & Padding overhead\\
\hline \hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{ l l l}
\hline \hline
$\slotind$ & \verb;\slotind; & Slot index IRSA\\
$\rateIrsa$ & \verb;\rateIrsa; & $1/\dg$ or rate in IRSA\\
$\ld$ & \verb;\ld; & Burst node edge perspective degree distribution\\
$\EBdegDist$ & \verb;\EBdegDist; & edge degree $\dg$ probability\\
$\Ld$ & \verb;\Ld; & Burst node node perspective degree distribution\\
$\BNdegDist$ & \verb;\BNdegDist; & node degree $\dg$ probability\\
$\davg$ & \verb;\davg; & Average user degree\\
$\dmax$ & \verb;\dmax; & Maximum user degree\\
$\rd$ & \verb;\rd; & Slot node edge perspective degree distribution\\
$\ESdegDist$ & \verb;\ESdegDist; & edge degree $\slotind$ probability\\
$\Rd$ & \verb;\Rd; & Slot node node perspective degree distribution\\
$\SNdegDist$ & \verb;\SNdegDist; & node degree $\slotind$ probability\\
$\thr$ & \verb;\thr; & Load threshold IRSA\\
$\exitb$ & \verb;\exitb; & Exit function\\
$\exits$ & \verb;\exits; & Exit function\\
$\p$ & \verb;\p; & Prob. of carrying an erasure message given it is connected to a \\
& & burst node of degree $\dg$\\
$\q$ & \verb;\q; & Prob. of carrying an erasure message given it is connected to a \\
& & slot node of degree $\slotind$\\
$\snr$ & \verb;\snr; & Received SNR value\\
$\snravg$ & \verb;\snravg; & Average received SNR value\\
$\snrrv$ & \verb;\snrrv; & SNR random variable\\
$\power$ & \verb;\power; & Received power\\
$\snrdist$ & \verb;\snrdist; & SNR distribution\\
$\powerdist$ & \verb;\powerdist; & Power distribution\\
$\zt$ & \verb;\zt; & $\zt=(1+\snrthr)^t$\\
$\calB$ & \verb;\calB; & Set of $\numUs$ user nodes\\
$\calS$ & \verb;\calS; & Set of $\numSlot$ slot nodes\\
$\slot$ & \verb;\slot; & Slot index\\
$\PLRtarget$ & \verb;\PLRtarget; & Target \ac{PLR}\\
$\sDegJ$ & \verb;\sDegJ; & Slot degree of slot $j$ at a certain iteration of\\
& & \ac{SIC} IRSA\\
$\decStep$ & \verb;\decStep; & Decoding step of intra-slot IC IRSA\\
\hline \hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{ l l l}
\hline \hline
$\ulVal$ & \verb;\ulVal; & Subscript for the uplink\\
$\dlVal$ & \verb;\dlVal; & Subscript for the downlink\\
$\loadMax$ & \verb;\loadMax; & Channel load corresponding to the max Throughput\\
$\tpMax$ & \verb;\tpMax; & Max Throughput\\
$\tpSA$ & \verb;\tpSA; & Throughput SA\\
$\tpUL$ & \verb;\tpUL; & Throughput in the uplink\\
$\tpULMax$ & \verb;\tpULMax; & Max Throughput in the uplink\\
$\tpULk{k}$ & \verb;\tpULk{k}; & Throughput at relay k in the uplink\\
$\tpULkMax{k}$ & \verb;\tpULkMax{k}; & Max Throughput at relay k in the uplink\\
$\tpDL$ & \verb;\tpDL; & Throughput donwlink\\
$\tpetoe$ & \verb;\tpetoe; & Throughput end-to-end\\
$\ulrk{k}$ & \verb;\ulrk{k}; & Prob. that the packet is not collected by any of the $\nrx$ relays\\
$\nrx$ & \verb;\nrx; & Number of relays\\
$\rxEl$ & \verb;\rxEl; & Relay index\\
$\collRV$ & \verb;\collRV; & r.v. of the number of columns in a matrix\\
$\coll$ & \verb;\coll; & Number of columns in a matrix\\
$\collMax$ & \verb;\collMax; & Max number of columns in a matrix\\
$\collK{k}$ & \verb;\collK{k}; & number of columns in a specific matrix $k$\\
$\colVec$ & \verb;\colVec; & uplink collected packets\\
$\colVecK{k}$ & \verb;\colVecK{k}; & uplink collected packets by relay $k$\\
$\linll$ & \verb;\linll; & Number of rows in a matrix\\
$\linllK{k}$ & \verb;\linllK{k}; & Number of rows in a matrix $k$\\
$\linComb$ & \verb;\linComb; & linear combinations built at the gateway\\
$\linCombK{k}$ & \verb;\linCombK{k}; & linear combinations built at the gateway from collected\\
& & packets at relay $k$\\
$\MxComb$ & \verb;\MxComb; & Matrix\\
$\MxCombTwo$ & \verb;\MxCombTwo; & Matrix two\\
$\MxCombK{k}$ & \verb;\MxCombK{k}; & Matrix $k$\\
\hline \hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{ l l l}
\hline \hline
$\fieldOrd$ & \verb;\fieldOrd; & finite field order\\
$\peras$ & \verb;\peras; & erasure probability in the uplink links\\
$\capDL$ & \verb;\capDL; & Downlink capacity\\
$\numulslot$ & \verb;\numulslot; & Number of uplink slots\\
$\mxNumCol$ & \verb;\mxNumCol; & Max number of columns\\
$\rank$ & \verb;\rank; & rank of the matrix\\
$\rankK{k}$ & \verb;\rankK{k}; & rank of the matrix $k$\\
$\rankKMax{k}$ & \verb;\rankKMax{k}; & Max. rank of matrix $k$\\
$\mxCol$ & \verb;\mxCol; & to set\\
$\mxColK{k}$ & \verb;\mxColK{k}; & to set\\
$\colNumVec$ & \verb;\colNumVec; & to set\\
$\evSlotSet$ & \verb;\evSlotSet; & countably infinite set of possible outcomes at slot $\slot$\\
$\evSlot$ & \verb;\evSlot; & given event in the set of outcomes in a slot\\
$\obsSlot$ & \verb;\obsSlot; & r.v. slot observation\\
$\setColPack$ & \verb;\setColPack; & the set of collected packets\\
$\setRel$ & \verb;\setRel; & the set of relays\\
$\setCommPack$ & \verb;\setCommPack; & the set of packets in common at the relays\\
$\carI$ & \verb;\carI; & cardinality of $\setCommPack$\\
$\evNotRx$ & \verb;\evNotRx; & event of not received packet by any receiver\\
$\dataPart$ & \verb;\dataPart; & $L$-bit data part of packet\\
$\dataSet$ & \verb;\dataSet; & $L$-bit data part of packet\\
$\obsPk$ & \verb;\obsPk; & Observed packets at gateway\\
$\obsPkTwo$ & \verb;\obsPkTwo; & Observed packets at gateway distinct packets\\
$\rateDw$ & \verb;\rateDw; & Downlink rate\\
$\erPos$ & \verb;\erPos; & All erasures positions\\
$\entropy$ & \verb;\entropy; & Entropy\\
$\Prob$ & \verb;\Prob; & Probability\\
$\setUnique$ & \verb;\setUnique; & Set of unique/distinct packets observed by the relays\\
$\setVar$ & \verb;\setVar; & Set of variables involved in less equations\\
$\setInterest$ & \verb;\setInterest; & Set of interest\\
$\eventInterest$ & \verb;\eventInterest; & Event of interest\\
$\rateDwSet$ & \verb;\rateDwSet; & Set of downlink rates\\
\hline \hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{ l l l}
\hline \hline
$\dropVec$ & \verb;\dropVec; & Dropping probability vector\\
$\drop$ & \verb;\drop; & Dropping probability\\
$\cardSpace$ & \verb;\cardSpace; & Cardinality of the space\\
$\coeffa$ & \verb;\coeffa; & First coefficient\\
$\coeffb$ & \verb;\coeffb; & Second coefficient\\
$\coeffc$ & \verb;\coeffc; & Third coefficient\\
$\coeffd$ & \verb;\coeffd; & Fourth coefficient\\
$\coeffe$ & \verb;\coeffe; & Fifth coefficient\\
\hline \hline
\end{tabular}
\end{center}

\clearpage 

==> sections/preamble.tex <==
\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}

\newcommand{\fede}[1]{\textcolor{red}{#1}}
\newcommand{\giangio}{\textcolor{blue!80}}
\newcommand{\andrea}{\textcolor{green!80}}

%%%% Notation

\newcommand{\ET}{\mathrm{E}_T}    %% Tx energy
\newcommand{\EL}{\mathrm{E}_L}    %% Listen energy
\newcommand{\EI}{\mathrm{E}_I}    %% Idle energy
\newcommand{\E}{\mathrm{E}}		  % % Total average energy


\newcommand{\La}{\Lambda}    %% Node oriented dd (user)
\newcommand{\Rh}{\mathrm{P}}    %% Node oriented dd (slot)
\newcommand{\la}{\lambda}    %% edge oriented dd (user)
\newcommand{\rh}{\rho}    %% egde oriented dd (slot)

\newcommand{\iLa}[1]{\Lambda^{(#1)}}    %% Induced Node oriented dd (user)
\newcommand{\iRh}[1]{\mathrm{P}^{(#1)}}    %% Induced  Node oriented dd (slot)
\newcommand{\ila}[1]{\lambda^{(#1)}}    %% Induced edge oriented dd (user)
\newcommand{\irh}[1]{\rho^{(#1)}}    %% Induced  egde oriented dd (slot)

\newcommand{\graph}{\mathscr{G}}    %% Graph
\newcommand{\uset}{\mathscr{U}}    %% user nodes set
\newcommand{\sset}{\mathscr{S}}    %% slot nodes set
\newcommand{\listset}{\mathscr{L}}    %% listen set
\newcommand{\sn}{\mathsf{s}}    %% listen set
\newcommand{\un}{\mathsf{u}}    %% listen set


\newcommand{\dum}{\mathtt{x}}    %% dummy variable

\newcommand{\load}{\mathsf{G}}    %% channel load
\newcommand{\thrp}{\mathsf{R}_{\mathrm{D}}}    %% throughput
\newcommand{\plr}{\mathsf{P}_{\mathrm{MD}}}    %% PLR

\newcommand{\thr}{\mathsf{G}^\star}    %% threshold
\newcommand{\plrt}{\plr^\star}    %% PLR

\newcommand{\slots}{n} % % number of slots per discovery phase
\newcommand{\tslot}{\mathrm{T}_s} % % number of slots per discovery phase
\newcommand{\users}{m} % % number of users in the network

\newcommand{\degree}{d} % % number of replicas sent per user, i.e. degree
\newcommand{\listn}{\ell} % % listening probability
\newcommand{\dmax}{{\degree_{\mathrm{max}}}}    %% Node oriented dd (user)
\newcommand{\avgd}{\bar\degree}    %% Node oriented dd (user)

\newcommand{\dcost}{\mathrm{D}_C}    %% Node oriented dd (user)


\newcommand\T{\rule{0pt}{2.6ex}}

